Computational Complexity of Traffic Hijacking under BGP and S-BGP

Harmful Internet hijacking incidents put in evidence how fragile the Border Gateway Protocol (BGP) is, which is used to exchange routing information between Autonomous Systems (ASes). As proved by recent research contributions, even S-BGP, the secure variant of BGP that is being deployed, is not fully able to blunt traffic attraction attacks. Given a traffic flow between two ASes, we study how difficult it is for a malicious AS to devise a strategy for hijacking or intercepting that flow. We show that this problem marks a sharp difference between BGP and S-BGP. Namely, while it is solvable, under reasonable assumptions, in polynomial time for the type of attacks that are usually performed in BGP, it is NP-hard for S-BGP. Our study has several by-products. E.g., we solve a problem left open in the literature, stating when performing a hijacking in S-BGP is equivalent to performing an interception.

==> Makefile <==
SHELL := /bin/bash

# Document title (extended)
DOCTITLE = 

# Directory containing document figures
FIGURES_DIRECTORY = figures
# Directory containing source files for document figures (must be inside the
# FIGURES_DIRECTORY
FIGURES_SOURCE_DIRECTORY = $(FIGURES_DIRECTORY)/source

# Directory containing bibliographic databases
BIBLIOGRAPHY_DIRECTORY = bibliography

# Directory containing files to be included
INCLUDE_DIRECTORY = include

# Main document name
MAIN_DOCUMENT = main

# The following variables contain the filenames of all the figures that can
# be rebuilt from a source file
FIGS = $(wildcard $(FIGURES_SOURCE_DIRECTORY)/*.fig)
PNGS = $(wildcard $(FIGURES_SOURCE_DIRECTORY)/*.png)
SOURCE_EPSES = $(wildcard $(FIGURES_SOURCE_DIRECTORY)/*.eps)
SOURCE_PDFS = $(wildcard $(FIGURES_SOURCE_DIRECTORY)/*.pdf)
SOURCE_PSTEXES = $(wildcard $(FIGURES_SOURCE_DIRECTORY)/*.pstex)


# $(EPSFIGS) contains the filenames of all the eps file derived from the figures
EPSFIGS= $(FIGS:%.fig=%.eps)



default: help

help:
	@echo
	@echo "Please choose the output to be produced..."
	@echo -e "\tmake dvi:   create a $(MAIN_DOCUMENT).dvi file"
	@echo -e "\tmake ps:    create a $(MAIN_DOCUMENT).ps file"
	@echo -e "\tmake pdf:   create a $(MAIN_DOCUMENT).pdf file"
	@echo "...or the operation to be performed"
	@echo -e "\tmake acroread: ensure document is up to date and show output using Acrobat Reader"
	@echo -e "\tmake gv:    ensure document is up to date and show output using gv"
	@echo -e "\tmake kdvi:  ensure document is up to date and show output using kdvi"
	@echo -e "\tmake xdvi:  ensure document is up to date and show output using xdvi"
	@echo -e "\tmake clean: delete all but source files"
	@echo
	@echo "Bibliography is automatically generated when needed."
	@echo "You don't need to run make more than once: cross references"
	@echo "are automatically rebuilt."
	@echo



BBL_DEPENDENCIES = $(wildcard $(BIBLIOGRAPHY_DIRECTORY)/*.bib) \
                   $(MAIN_DOCUMENT).tex \
                   $(wildcard $(INCLUDE_DIRECTORY)/*.tex)
SOURCE_DEPENDENCIES = $(MAIN_DOCUMENT).tex \
                      $(MAIN_DOCUMENT).bbl \
                      $(wildcard $(INCLUDE_DIRECTORY)/*.tex)

epsfigs:
	for i in $(SOURCE_PSTEXES); do T="pstexTMPFILE"; FIGNAME=`basename "$${i%.pstex}"`; tmpFile="`mktemp $$T-XXXXXX`"; echo "\documentclass{article} \
		\usepackage{epsfig} \
		\usepackage{color} \
		\usepackage{amsfonts,amsmath,amssymb} \
		\setlength{\MUHAtextwidth}{100cm} \
		\setlength{\MUHAtextheight}{100cm} \
		\MUHAbegin{document} \
		\pagestyle{empty} \
		\input{$(FIGURES_DIRECTORY)/$$FIGNAME.pstex_t} \
		\end{document}" | sed 's/MUHA//g' > "$$tmpFile"; FSD="$(FIGURES_DIRECTORY)/"; SUBST="$${FSD//\//\\/}" ; echo "SUBST: $$SUBST"; sed "s/graphics{/graphics{$$SUBST/" $(FIGURES_SOURCE_DIRECTORY)/$$FIGNAME.pstex_t > $(FIGURES_DIRECTORY)/$$FIGNAME.pstex_t; cp "$$i" $(FIGURES_DIRECTORY); latex "$$tmpFile"; dvips -E "$$tmpFile.dvi" -o "$(FIGURES_DIRECTORY)/$$FIGNAME.eps"; rm $$T*; done
	for i in $(SOURCE_EPSES); do cp --no-preserve=mode "$$i" "$(FIGURES_DIRECTORY)"; done; chmod -R +w "$(FIGURES_DIRECTORY)" 
	for i in $(SOURCE_PDFS); do FIGNAME=`basename "$${i%.pdf}"`; if [ "$$i" -nt "$(FIGURES_DIRECTORY)/$$FIGNAME.eps" -o ! -e "$(FIGURES_DIRECTORY)/$$FIGNAME.eps" ]; then pdftops -eps "$$i" "$(FIGURES_DIRECTORY)/$$FIGNAME.eps"; fi; done
	for i in $(FIGS); do FIGNAME=`basename "$${i%.fig}"`; if [ "$$i" -nt "$(FIGURES_DIRECTORY)/$$FIGNAME.eps" -o ! -e "$(FIGURES_DIRECTORY)/$$FIGNAME.eps" ]; then fig2dev -L eps "$$i" "$(FIGURES_DIRECTORY)/$$FIGNAME.eps"; fi; done
	for i in $(PNGS); do FIGNAME=`basename "$${i%.png}"`; if [ "$$i" -nt "$(FIGURES_DIRECTORY)/$$FIGNAME.eps"  -o ! -e "$(FIGURES_DIRECTORY)/$$FIGNAME.eps" ]; then convert "$$i" "eps2:$(FIGURES_DIRECTORY)/$$FIGNAME.eps"; fi; done
	

pdffigs:
	for i in $(SOURCE_PSTEXES); do T="pstexTMPFILE"; FIGNAME=`basename "$${i%.pstex}"`; tmpFile="`mktemp $$T-XXXXXX`"; echo "\documentclass{article} \
		\usepackage{epsfig} \
		\usepackage{color} \
		\setlength{\MUHAtextwidth}{100cm} \
		\setlength{\MUHAtextheight}{100cm} \
		\MUHAbegin{document} \
		\pagestyle{empty} \
		\input{$(FIGURES_DIRECTORY)/$$FIGNAME.pstex_t} \
		\end{document}" | sed 's/MUHA//g' > "$$tmpFile"; FSD="$(FIGURES_DIRECTORY)/"; SUBST="$${FSD//\//\\/}" ; echo "SUBST: $$SUBST"; sed "s/graphics{/graphics{$$SUBST/" $(FIGURES_SOURCE_DIRECTORY)/$$FIGNAME.pstex_t > $(FIGURES_DIRECTORY)/$$FIGNAME.pstex_t; cp "$$i" $(FIGURES_DIRECTORY); latex "$$tmpFile"; dvips -E "$$tmpFile.dvi" -o "$(FIGURES_DIRECTORY)/$$FIGNAME.eps"; epstopdf "$(FIGURES_DIRECTORY)/$$FIGNAME.eps" --outfile="$(FIGURES_DIRECTORY)/$$FIGNAME.pdf"; rm $$T*; done	
	for i in $(SOURCE_EPSES); do FIGNAME=`basename "$${i%.eps}"`; if [ "$$i" -nt "$(FIGURES_DIRECTORY)/$$FIGNAME.pdf" -o ! -e "$(FIGURES_DIRECTORY)/$$FIGNAME.pdf" ]; then epstopdf "$$i" --outfile="$(FIGURES_DIRECTORY)/$$FIGNAME.pdf"; fi; echo $$FIGNAME; done
	for i in $(SOURCE_PDFS); do cp --no-preserve=mode "$$i" "$(FIGURES_DIRECTORY)"; done; chmod -R +w "$(FIGURES_DIRECTORY)" 
	for i in $(FIGS); do FIGNAME=`basename "$${i%.fig}"`; if [ "$$i" -nt "$(FIGURES_DIRECTORY)/$$FIGNAME.pdf"  -o ! -e "$(FIGURES_DIRECTORY)/$$FIGNAME.pdf" ]; then fig2dev -L pdf "$$i" "$(FIGURES_DIRECTORY)/$$FIGNAME.pdf"; fi; done
	for i in $(PNGS); do FIGNAME=`basename "$${i%.png}"`; if [ "$$i" -nt "$(FIGURES_DIRECTORY)/$$FIGNAME.pdf"  -o ! -e "$(FIGURES_DIRECTORY)/$$FIGNAME.pdf" ]; then convert "$$i" "$(FIGURES_DIRECTORY)/$$FIGNAME.pdf"; fi; done


# Cancel implicit rule for dvi files
%.dvi: %.tex

$(MAIN_DOCUMENT).bbl: $(BBL_DEPENDENCIES) epsfigs
	latex $(MAIN_DOCUMENT).tex
	bibtex $(MAIN_DOCUMENT)

dvi: $(MAIN_DOCUMENT).dvi 

$(MAIN_DOCUMENT).dvi: $(SOURCE_DEPENDENCIES) epsfigs
# Several runs are required in order to get cross-references and
# changebars right
	latex $(MAIN_DOCUMENT).tex
	latex $(MAIN_DOCUMENT).tex >/dev/null
	latex $(MAIN_DOCUMENT).tex >/dev/null

ps: $(MAIN_DOCUMENT).ps

$(MAIN_DOCUMENT).ps: $(MAIN_DOCUMENT).dvi
	dvips $(MAIN_DOCUMENT).dvi -o $(MAIN_DOCUMENT).ps
	@echo -e ',s/\\(%%Title: \\).*/\\1$(DOCTITLE)/\nw' | ed $(MAIN_DOCUMENT).ps

pdf: $(MAIN_DOCUMENT).pdf 

$(MAIN_DOCUMENT).pdf: $(SOURCE_DEPENDENCIES) pdffigs
# Several runs are required in order to get cross-references and
# changebars right
	pdflatex $(MAIN_DOCUMENT).tex
	pdflatex $(MAIN_DOCUMENT).tex >/dev/null
	pdflatex $(MAIN_DOCUMENT).tex >/dev/null
	pdflatex $(MAIN_DOCUMENT).tex >/dev/null



acroread: pdf
	acroread $(MAIN_DOCUMENT).pdf

gv: ps
	gv $(MAIN_DOCUMENT).ps

xdvi: dvi
	xdvi -s 3 $(MAIN_DOCUMENT).dvi

kdvi: dvi
	kdvi $(MAIN_DOCUMENT).dvi



clean:
	-rm $(wildcard *~ *.cb* *.log *.aux *.toc *.dvi *.bbl *.blg *.lof *.lot *.out *.ps *.pdf *.backup) \
       $(wildcard $(INCLUDE_DIRECTORY)/*.aux $(FIGURES_DIRECTORY)/*.eps \
       $(FIGURES_DIRECTORY)/*.pdf $(FIGURES_DIRECTORY)/*.pstex*) >/dev/null


==> plain_bgp.tex <==


% ------------------------------------------------------------------
\section{Checking if a Plain BGP Attack Exists}\label{sect:plain-bgp}
% \section{Complex Attacks are still Easy to Check if no BGP Security Mechanism Is Adopted}\label{sect:plain-bgp}
% \section{Plain BGP}\label{sect:plain-bgp}
% ------------------------------------------------------------------

In this section, we show that, in general, it is hard to find an attack strategy (Theorem~\ref{theo:grexpall_no_asset_ndb_bgp}), while the problem turns to be easier in a more realistic setting (Theorem~\ref{theo:grexpall_no_asset_plb_bgp}). 

%
% DEFINITION AND NOTATION 
%
We introduce some notation. A \emph{ranking function} determines the level of preference of paths available at vertex $v$. If $P_1, P_2$ are available at $v$ and $P_1$ is \emph{preferred} over $P_2$ we write $P_1<_\lambda^v P_2$.
%
The \emph{concatenation} of two nonempty paths $P=(v_k\ v_{k-1}\ \dots\ v_j)$, $k \geq j$, and $Q=(v_i\ v_{i-1}\ \dots\ v_0)$, $i \geq 0$, denoted as $PQ$, is the path $(v_k\ v_{k-1}\ \dots\ v_{j-1}\ v_i\ v_{i-1}\ \dots\ v_0)$ if $v_i=v_j$, otherwise $(v_k\ v_{k-1}\ \dots\ v_j\ v_i\ v_{i-1}\ \dots\ v_0)$.
%
Also, let $P$ be a valley-free path from vertex $v$. We say that $P$ \emph{is of class} $3$, $2$, or $1$ if it traverses a customer, a peer, or a provider of $v$, respectively. We also define a function $f^v$ for each vertex $v$, that maps each path from $v$ to the integer of its class. Given two paths $P$ and $P'$ available at $v$ if $f^v(P)>f^v(P')$ we say that the class of $P$ \emph{is better than} the class of $P'$.
%
In stable routing state $S$, a path $P=(v_1\ \dots\ v_n)$ is \emph{disrupted at vertex} $v_i$ by a path $P'$ if there exists a vertex $v_i$ of $P$ such that $v_i$ selects path $P'$.
%  over $(v_i\ \dots\ v_n)$ and selects $P'$ and (ii) $v_{i+1}$ selects $(v_{i+1}\ \dots\ v_n)$.
%
Also, if $P'$ is preferred over $(v_i\ \dots\ v_n)$ because of the GR3 condition, we say that path $P$ \emph{is disrupted by a path of a better class}. 
%
Otherwise, if $P'$ is preferred over $(v_i\ \dots\ v_n)$ because of the shortest-paths criterion, we say that  $P$ is disrupted by a path of the \emph{same class}. 


An hijacking can be obviously found in exponential time by a simple
brute force approach which simulates every possible attack strategy and
verifies its effectiveness. The exponential complexity of this approach is due to two
factors: (i) even in the case when a single path is announced, $m$ has
to decide to what neighbors the announcement is sent, which results in
an exponential number of possibilities w.r.t.\ the number of neighbors;
(ii) in the case $m$ has \plainBgp capabilities, a single announcement
can be forged in an exponential number of ways w.r.t.\ the number of
vertices of the graph. Hence, the following result in the case the Internet graph has no bound constraints may be not surprising at all.

\newcommand{\greBgpNoAssetNdb}{
If the manipulator has \plainBgp cheating capabilities 
%removed bounded degree column% and the degree of the manipulator's vertex is bounded by a constant $k$, 
then problem \hijack is \NPhard. 
}

\begin{theorem}\label{theo:grexpall_no_asset_ndb_bgp}
\greBgpNoAssetNdb
\end{theorem}

Surprisingly, in a more realistic scenario, where the length of the valley-free paths is bounded by a constant $k$, we have that in the \plainBgp setting an attack strategy can be found in polynomial time.

% BRIEF EXPLANATION POLYTIME ALGORITHM PLAIN BGP

% A polynomial time algorithm can be designed exploiting two intuitions that will be proved below.
% First, a manipulator $m$ has no benefit in announcing paths longer than
% $k$. This removes the exponential complexity of factor (ii). If
% there exists an attack strategy that allows $m$ to attract traffic from
% $s$ through a path $P$ announced to the neighbor of $m$,
% then the attack still works if $m$ announces to each of its neighbors,
% except $n$, a faked path that contains every vertex in $P$, except $s$,
% and announces to $n$ a simple path containing only vertex $m$. Exploiting this
% second intuition allows to remove the exponential complexity of
% factor (i).

\newcommand{\greBgpPlainPlb}{
If the manipulator has \plainBgp cheating capabilities and the length of the longest valley-free path is at most $k$, 
%removed bounded degree column% and the degree of the manipulator's vertex is bounded by a constant $k$, 
then problem \hijack is \NPhard. 
}

\begin{theorem}\label{theo:grexpall_no_asset_plb_bgp}
\greBgpPlainPlb
\end{theorem}

\begin{proof}
 See Fig.~\ref{fig:bgp_plain_plb_hard}. The only path shorter than the one contained in the \longLengthStruct is the one in the \intLengthStruct. Hence, $m$ should announce to $j_1$ that it is the originator of prefix $\pi$. Also, $m$ has to disrupt every path contained in the \shoLengthStruct. To do this, $m$ have to announce something to its neighbors $n_1,\dots,n_t$. Consider variable $X_i$. It exists a path $P_{w_id}$ from $w_i$ to $d$ such that, if it is selected at $w_i$, it disrupts the path in the \intLengthStruct by better class. Hence, $m$ should announce something to neighbor $n_i$ in order to be selected at vertex $w_i$. Of course, in such announcement $m$ should include vertex $j_1$, otherwise it disrupts the path in the \intLengthStruct with a longer path. Since vertex $w_i$ discriminates its selection by the same class, $m$ should announce a path that is shorter than or equal to $p_{w_id}$. Path $p_{w_id}$ has length $7$.
\begin{figure}[t]
% \centering
\begin{minipage}[t]{0.49\textwidth}%
% \vspace{0.3in}
\includegraphics[width=1\textwidth]{figures/bgp_plain_plb_hard}
\caption{Reduction of \threesat problem to the \hijack problem when $m$ has \plainBgp capabilities and the length of the longest valley-free path is at most $k$.}\label{fig:bgp_plain_plb_hard}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.49\textwidth}%
\includegraphics[width=1\textwidth]{figures/bgp_sbgp_plb_grexpall_new}
\caption{Reduction of a constrained \threesat problem to the \hijack problem when $m$ has \SBGP cheating capabilities.}\label{fig:bgp_sbgp_plb_grexpall}
\end{minipage}
\end{figure}

\end{proof}





% % % % % % % % % % OLD WRONG PLAIN BGP ALGORUITHM % % % % % % % % % % % % 
\remove{
We introduce the following structural lemma.

% Theorem~\label{theo:grexpall_no_asset_plb_bgp} is based on the following idea, supported by Lemma~\ref{lemma:grexpall_plain_better_class_disruption}. 

% % % % % ATTEMPT TO UNIFY LEMMA % % % % % 

Let $a^*$ be a successful attack of $m$ and let $a^*_s$ be the path selected by $s$.
We say that $a^*$ is the \emph{most preferred} successful attack if for each successful attack $a$ of $m$, where $a_s$ is the path selected by $s$, we have $a^*_s <_\lambda^s a_s $.

\newcommand{\lemmaAbsenceOfHigherValleyFreePath}{
Consider the most preferred successful attack for $m$ and let $p_{sm}q^l$ be the path that $s$ selects. 
It does not exists a valley-free path from $s$ to $d$ and not passing through $m$ in $G$ of class higher than $f^s(p_{sm}q^l)$.}

\begin{lemma}\label{lemma:grexpall_plain_absence_higher_valley_free_path}
\lemmaAbsenceOfHigherValleyFreePath
\end{lemma}

\begin{proof}
Suppose by contradiction that such path exists. Let $p_{sd}$ be the shortest valley-free path from $s$ to $d$ among those paths from $s$ to $d$ of the highest possible class (tie breaks are resolved arbitrarily). Let $n$ be the neighbor of $s$ in $p_{sd}$ and $p_{nd}$ be the subpath from $n$ to $d$ of $p_{sd}$.
Observe that, $n$ cannot be a provider of $s$ because $f^s(p_{sd})>f^s(p_{sm}q^l)$.
Since $n$ is a peer or a customer of $s$, we have that $p_{nd}$ is a directed path from $d$ to $n$. By GR1 condition, each directed path is simple. Observe that $p_{nd}$ should be disrupted by $m$ otherwise it is available at $s$. But it implies that there exists at least a valley-free path $p_{sm}^*$ between $m$ and $s$ of class $f^s(p_{sd})$. Now, consider an attack for $m$, where $m$  announces $(d)$ to $n_j$, where $n_j$ is the vertex adjacent to $m$ in $p_{sm}^*$, and it announces $\epsilon$ to the rest of its neighbors. Since $p_{sm}^*$ can be disrupted only by a shorter path directed to $m$ and it can be disrupted by better class only at $s$, we have that $n$ selects a path to $m$ and so also $s$ has an available path preferred over $p_{sm}q^l$. That is a contradiction. 
\qed
\end{proof}

\newcommand{\lemmaAbsenceOfSameValleyFreePath}{
Consider the most preferred successful attack for $m$. Let $p_{sm}q^l$ be the path that $s$ selects. Each path $p$ of class  $f^s(p_{sm}q^l)$ from $s$ to $d$ such that $p <_\lambda^s p_{sm}q^l$ is disrupted by better class.}

\begin{lemma}\label{lemma:grexpall_plain_absence_same_valley_free_path}
\lemmaAbsenceOfSameValleyFreePath
\end{lemma}

\begin{proof}
Suppose by contradiction that there exists a valley-free path $p$ such that $p <_\lambda^s p_{sm}q^l$ and $p$ is not disrupted by better class. If $p$ is not disrupted by $m$, we have a contradiction since a path 
\end{proof}

\newcommand{\lemmaEasyDisruptionBetterClass}{
Consider the best successful attack $<q^1,\dots,q^t>$ for $m$. Let $p_{sm}q^l$ be the path selected at $s$. Let $v$ be a vertex such that it selects a path $p$ from a customer (peer). 
If $m$ adopts attack $<\bar q^1  , \dots,\bar q^t>$, where $\bar q^i=p_{sm}$ for $i=1,\dots,l-1,l+1,\dots,t$, and $\bar q^l=q^l$, then $v$  selects a path from a customer (peer) and $s$ selects $p_{sm}q^l$.
}

\begin{lemma}\label{lemma:grexpall_plain_easy_disruption_better_class}
  \lemmaEasyDisruptionBetterClass
\end{lemma}

\begin{proof}
Consider strategy $S$. 
If $f^v(p)=3$, let $U_v$ be the set of all directed paths from $d$ to $v$.  Moreover, for every neighbor $n_i$ of $m$, for every directed path $p_{vn_i}$ from $n_i$ to $v$, if $q_{mi}\neq \epsilon$, where $q_{mi}$ is the path announced from $m$ to $n_i$, then add path $p_{vn_i}q_{mi}$ to $U$ if it is simple. Let $p^c_v$ be the shortest path in $U$. Such path is selected at $v$ because there does not exist any shorter path that can disrupt it. Then,  $p^c_v=p$. 

Now, if $m$ announces $(d)$ to $n_l$,  we consider two cases: $p$ is originated by $d$, or not. In the first case,  $p$ cannot be disrupted since it is the shorter path. In the second case, we have that $|p_{vn_l}(d)|\le|p_{vn_l}q_{ml}|$, which implies that path $p_{vn_l}(d)$ is selected at $v$ and the statement is proved in that case.

Otherwise, if $f^v(p_{vn_l}q_{ml})=2$, we consider strategy $s$ and for each peer $r$ of $v$ we define path $p^c_r$ as above. By Lemma~\ref{lemma:grexpall_plain_absence_higher_valley_free_path}, there does not exist any valley-free path $p$ from $v$ to $d$ such that $f^v(p)>f^v(p_{vn_l}q_{ml})$ and any $p^c_r$ path passes through $v$. As before, each $p^c_r$ is selected at $r$ because it is the shortest possible directed path to $r$. Let $r^*$ be a peer of $v$ such that $p^c_{r^*}$ is the shortest possible directed path. Then $p_{vn_l}q_{ml}=(v\ r^*)p^c_{r^*}$.
Now, if $m$ announces $(d)$ to $n_l$, we have that $|p_{vn_l}(d)|\le|p_{vn_l}q_{ml}|$, which implies that path $p_{vn_l}(d)$ is selected at $v$ and the statement is proved also in that case.
\qed
\end{proof}

\newcommand{\lemmaLongerPathClass}{
 Consider a successful attack for $m$. Let $p_{sm}q^l$ be the path selected at $s$. Suppose that for every valley-free path $p$ between $s$ and $d$ such that $f^s(p_{sm}q^l)=f^s(p)$, $p <_\lambda^s p_{sm}q^l$ holds.
If $m$ adopts attack $A=<\bar q^1  , \dots,\bar q^t>$, where $\bar q^i=q^i$ for $i=1,\dots,l-1,l+1,\dots,t$, and $\bar q^l=(d)$, then $A$ is successful.
}

\begin{lemma}\label{lemma:grexpall_plain_easy_disruption_better_class}
  \lemmaLongerPathClass
\end{lemma}

\begin{proof}
 \dots
\end{proof}



\newcommand{\lemmaSameClassPathDisruptionBetterClass}{
Consider a successful strategy for $m$. Let $p_{sm}q_{ml}$ be the path that $s$ selects. 
Let $p_s=(v_1\ \dots\ v_t)$ be a valley-free path from $s$ to $d$ such that $p_s <_\lambda^s p_{sm}q_{ml}$.
At least a vertex $v_i$ of $p_s$ selects a path $p_{v_i}$  such that $f^{v_i}(p_{v_i})>f^{v_i}((v_i\ \dots\ v_t))$.
}

\vspace{2mm}
\begin{lemma}\label{lemma:grexpall_plain_same_class_path_disruption_better_class}
\lemmaSameClassPathDisruptionBetterClass
\end{lemma}
\vspace{2mm}

\begin{proof}
%  By Lemma~\ref{lemma:grexpall_plain_absence_higher_valley_free_path} we have that $f^s(p_s)=f^s(p_{sm}q_{ml})$. Suppose the statement does not hold, each vertex $v_i$ of $p_s$ selects a path $p_{v_i}$ such that $|p_{v_i}|\le|(v_i\ \dots\ v_t)|$. Such path $p_{v_i}$ does not contain any vertex $v_k$ in $\{v_1\ \dots\ v_{i+1}\}$, otherwise $v_k$ selects a path $p_{v_k}$ such that $f^s(p_{v_k})>f^s((v_k\ \dots\ v_t))$, that is a contradiction. Hence, $s$ receives a path shorter than $p_s$, that is preferred over $p_{sm}q_{ml}$, which leads to a  contradiction. 
%  \qed
 By Lemma~\ref{lemma:grexpall_plain_absence_higher_valley_free_path} we have that $f^s(p_s)=f^s(p_{sm}q_{ml})$. Suppose the statement does not hold, each vertex $v_i$ of $p_s$ selects a path $p_{v_i}$ such that $|p_{v_i}|\le|(v_i\ \dots\ v_t)|$. Such path $p_{v_i}$ does not contain any vertex $v_k$ in $\{v_1\ \dots\ v_{i+1}\}$, otherwise $v_k$ selects a path $p_{v_k}$ such that $f^s(p_{v_k})>f^s((v_k\ \dots\ v_t))$, that is a contradiction. Hence, $s$ receives a path shorter than $p_s$, that is preferred over $p_{sm}q_{ml}$, which leads to a  contradiction. 
 \qed
\end{proof}




% % % % %  END ATTEMPT TO UNIFY LEMMAS % % % % %

\newcommand{\lemmaDisruptedByBetterClass}{
Consider a successful strategy for $m$. Let $P_m$ be the path that $s$ selects. Suppose it is the shortest among all the successful strategies of $m$.
Let $P_s$ be a valley-free path from $s$ to $d$ such that $P_s <_\lambda^s P_m$ and $P_s$ is not disrupted by a path through $d$ of better class. Path $P_s$ is disrupted by a path through $m$ of better class.}

\vspace{2mm}
\begin{lemma}\label{lemma:grexpall_plain_better_class_disruption}
\lemmaDisruptedByBetterClass
\end{lemma}
\vspace{2mm}

\begin{proof}
Suppose by contradiction that there exists at least a valley-free path $P_s$ from $s$ to $d$ such that $P_s <_\lambda^s P_m$, $P_s$ is not disrupted by a path through $d$ of better class, and either (i) $P_s$ is disrupted by a path through $m$ of same  class or (ii) $P_s$ is not disrupted at all.
% 
If (i), we have a contradiction since $s$ receives a path $P^*_s$ such that $|P^*_s|\le|P_s|$ that is preferred over $P_m$.
If (ii), since path $P_s$ is preferred over $P_m$, we have a contradiction because $s$ selects $P_s$. 
\end{proof}




\newcommand{\greBgpNoAssetPlb}{
If the manipulator has \plainBgp cheating capabilities and the length of
the longest valley-free path is at most $k$, then problem \hijack is
in P.}

\begin{theorem}\label{theo:grexpall_no_asset_plb_bgp}
\greBgpNoAssetPlb
\end{theorem}

\begin{algorithm}[h!]
\caption{Algorithm for the \hijack problem where $m$ has \plainBgp capabilities and the longest valley-free path in the graph is bounded by a constant $k$.}
\label{algo:bgp_no_asset_plb_grexpall}
\algsetup{indent=2em}
\begin{algorithmic}[1]
\STATE let $P_{sm}$ be the set of all valley-free paths from $s$ to $m$; 
\FORALL  { $p_{sm}$ in $P_{sm}$ }
 \STATE let $w$ be the vertex of $p_{sm}$ adjacent to $m$; remove from $p_{sm}$ both $s$ and $m$; let $N$ be the set of all neighbors of $m$ but $w$; let $Q$ be the set of all sets of vertices of $V \setminus \{m\}$ with at most $k$ vertices
 \FORALL {$q$ in $Q$}
%   \STATE let $A$ and $B$ be two empty paths; add to $A$, in any order, all vertices of $q$; add to $B$, in any order, all vertices in $p_{sm}$ except $s$
  \IF {the attacks succeeds when $m$ announces $q$ to $w$ and $p_{sm}$ to the vertices in $N$} 
   \RETURN $q$, $p_{sm}$, $w$
  \ENDIF 
 \ENDFOR
\ENDFOR
\RETURN fail
\end{algorithmic}
\end{algorithm}


\begin{proof}
We tackle the problem with Alg.~\ref{algo:bgp_no_asset_plb_grexpall}. 
%  
First, observe that line 6 tests if a certain set of announcements causes a successful attack and in case it returns the corresponding announcements. Hence, if Alg.~\ref{algo:bgp_no_asset_plb_grexpall} returns without failure it is trivial to see that it found a successful attack. 

Suppose now that there exists an attack strategy from $m$ that causes the attraction of traffic from $s$ and that is not found by Alg.~\ref{algo:bgp_no_asset_plb_grexpall}. If more than one such strategies exists, consider, w.l.o.g., the one in which $s$ selects a certain path $p$ such that $|p|$ is minimized. Denote by $n_1, \dots, n_j$ the neighbors of $m$ and by $q_{mi}$ the path announced from $m$ to $n_i$ in such a strategy. 
Let $p=p_{sm}q_{ml}$, where $p_{sm}$ is a valley-free path from $s$ to $m$. Path $q_{ml}$ is the (non necessarily valley-free) path announced by $m$ to the vertex $n_l$ adjacent to $m$ in $p_{sm}$.
Since the attack succeeds, $m$ announces to each of $n_1,\dots,n_{l-1},n_{l+1},\dots,n_j$ a path that does not disrupt $p_{sm}$.

Now we prove that $|p_{sm}q_{ml}| \leq k$. Suppose, for a contradiction, that $|p_{sm}q_{ml}| > k$. 
By Lemma~\ref{lemma:grexpall_plain_absence_higher_valley_free_path}, it does not exist any valley-free path from $s$ to $d$ of class higher than  $f^s(p_{sm}q_{ml})$ that passes through $m$.
% % % %  correct since here
Moreover, by Lemma~\ref{lemma:grexpall_plain_better_class_disruption}  each path $p_s$ from $s$ to $d$ such that  $p_s <_\lambda^s p_{sm}q_{ml}$ is disrupted at a vertex $u$ by a path $p_uq_{mt}$ through $m$ of better class, where $t$ is the neighbor of $m$ in $p_u$. Hence, $p_u$ excluding $u$ is a directed path from $m$.
Then, since $p_u$ cannot be disrupted by better class, except at $u$, if $m$ uses the \simpleHijack\footnote{why does simplehijack suffice?} attack, then every path preferred over $p_{sm}$ is disrupted and the hijack attack succeeds. In fact, $s$ select $p_{sm}$ as its best path. But this is a contradiction since $|p_{sm}|\le k$. Then, $|p_{sm}q_{ml}|\leq k$.

Then, since $p_u$ cannot be disrupted by better class, except at $u$, if $m$ uses the \simpleHijack attack, then every path preferred over $p_{sm}$ is disrupted and the hijack attack succeeds. In fact, $s$ select $p_{sm}$ as its best path. But this is a contradiction since $|p_{sm}|\le k$. Then, $|p_{sm}q_{ml}|\leq k$.

By Lemma~\ref{lemma:grexpall_plain_better_class_disruption}, each path $p_s$ from $s$ to $d$ such that  $p_s <\_lambda^s p_{sm}q_{ml}$  is disrupted at vertex $u$ by a path $p_u$ to $m$ of better class. Then, since $p_u$ cannot be disrupted by better class, except at $u$, if $m$ announces $q_{ml}$ to $n_l$ and $p_{sm}$ to neighbors  $n_1,\dots,n_{l-1},n_{l+1},\dots,n_j$, then $m$ still hijacks traffic from $s$. 
Since Alg.~\ref{algo:bgp_no_asset_plb_grexpall} can find the above strategy of attack we have a contradiction.

Finally, since the size of the sets is bounded by a constant, the cycle of the algorithm where all sets are considered requires a number of iterations that is polynomial in the number of vertices of the graph. Also, the disruption checks can be performed in polynomial time by using the algorithm in~\cite{ssz-ssir-09}.
\qed
\end{proof}


}
